Modal Logic and the Approximation Induction Principle

We prove a compactness theorem in the context of Hennessy-Milner logic. It is used to derive a sufficient condition on modal characterizations for the Approximation Induction Principle to be sound modulo the corresponding process equivalence. We show that this condition is necessary when the equivalence in question is compositional with respect to the projection operators.

==> eptcsdata.tex <==
\providecommand{\event}{S.~Fr\"oschle, D.~Gorla (Eds.): Workshop on Expressiveness\\
in Concurrency 2009 (EXPRESS'09).}
\providecommand{\volume}{8}
\providecommand{\anno}{2009}
\providecommand{\firstpage}{41}
\providecommand{\eid}{4}
\pdfoutput=1

